Graph Learning for Planning: The Story Thus Far and Open Challenges

Graph learning is naturally well suited for use in planning due to its ability to exploit relational structures exhibited in planning domains and to take as input planning instances with arbitrary number of objects. In this paper, we study the usage of graph learning for planning thus far by studying the theoretical and empirical effects on learning and planning performance of (1) graph representations of planning tasks, (2) graph learning architectures, and (3) optimisation formulations for learning. Our studies accumulate in the GOOSE framework which learns domain knowledge from small planning tasks in order to scale up to much larger planning tasks. In this paper, we also highlight and propose the 5 open challenges in the general Learning for Planning field that we believe need to be addressed for advancing the state-of-the-art.

==> figures/proofs/asnets-ilg.tex <==
\newcommand{\xxshift}{1.25cm}
\newcommand{\yyshift}{2cm}
\newcommand{\csize}{0.8cm}
\newcommand{\descccsize}{\scriptsize}
\newcommand{\objectsize}{\descccsize}
\newcommand{\ilgword}[1]{\text{\descccsize{#1}}}
\newcommand{\objword}[1]{\text{\objectsize{#1}}}
\newcommand{\desccccc}{5cm}
\newcommand{\desccc}{6cm}
\newcommand{\anchor}{west}
\newcommand{\minimumheight}{1.5em}
\centering
\begin{subfigure}{0.49\columnwidth}
    \centering
    \begin{tikzpicture}[
            thick,
            every node/.style={
                    % shape=circle,
                    % minimum size=\csize,
                    % align=center,  
                    draw,
                    rounded corners,
                    minimum height=\minimumheight,  % Adjust as needed  
                    % minimum width=2cm,   % Adjust as needed  
                }
        ]
        \node[fill=caribbeangreen] (onaa) at (-2.25*\xxshift,\yyshift) {
            $\ilgword{Q(a,a)}$
        };
        \node[fill=caribbeangreen] (onbb) at (-0.75*\xxshift,\yyshift) {
            $\ilgword{Q(b,b)}$
        };
        \node[fill=yellow] (onab) at ( 0.75*\xxshift,\yyshift) {
            $\ilgword{W(a,b)}$
        };
        \node[fill=yellow] (onba) at ( 2.25*\xxshift,\yyshift) {
            $\ilgword{W(b,a)}$
        };
        \node[fill=babyblue] (a) at (  -1.5*\xxshift,2*\yyshift) {
            $\objword{a}$
        };
        \node[fill=babyblue] (b) at (   1.5 *\xxshift,2*\yyshift) {
            $\objword{b}$
        };

        \path [-,draw=plta] (a.south) edge[bend left=15] (onaa.north);
        \path [-,draw=pltb] (a.south) edge[bend right=15] (onaa.north);
        \path [-,draw=plta] (b.south) edge[bend left=15] (onbb.north);
        \path [-,draw=pltb] (b.south) edge[bend right=15] (onbb.north);

        \path [-,draw=plta] (a.south) edge (onab.north);
        \path [-,draw=pltb] (b.south) edge (onab.north);

        \path [-,draw=plta] (b.south) edge (onba.north);
        \path [-,draw=pltb] (a.south) edge (onba.north);

    \end{tikzpicture}
    \caption{\subcapa}
\end{subfigure}
\begin{subfigure}{0.49\columnwidth}
    \centering
    \begin{tikzpicture}[
            thick,
            every node/.style={
                    % shape=circle,
                    % minimum size=\csize,
                    % align=center,  
                    draw,
                    rounded corners,
                    minimum height=\minimumheight,  % Adjust as needed  
                    % minimum width=2cm,   % Adjust as needed  
                }
        ]
        \node[fill=caribbeangreen] (onaa) at (-2.25*\xxshift,\yyshift) {
            $\ilgword{Q(a,b)}$
        };
        \node[fill=caribbeangreen] (onbb) at (-0.75*\xxshift,\yyshift) {
            $\ilgword{Q(b,a)}$
        };
        \node[fill=yellow] (onab) at ( 0.75*\xxshift,\yyshift) {
            $\ilgword{W(a,b)}$
        };
        \node[fill=yellow] (onba) at ( 2.25*\xxshift,\yyshift) {
            $\ilgword{W(b,a)}$
        };
        \node[fill=babyblue] (a) at (  -1.5*\xxshift,2*\yyshift) {
            $\objword{a}$
        };
        \node[fill=babyblue] (b) at (   1.5 *\xxshift,2*\yyshift) {
            $\objword{b}$
        };

        \path [-,draw=plta] (a.south) edge (onaa.north);
        \path [-,draw=pltb] (b.south) edge (onaa.north);
        \path [-,draw=plta] (b.south) edge (onbb.north);
        \path [-,draw=pltb] (a.south) edge (onbb.north);

        \path [-,draw=plta] (a.south) edge (onab.north);
        \path [-,draw=pltb] (b.south) edge (onab.north);

        \path [-,draw=plta] (b.south) edge (onba.north);
        \path [-,draw=pltb] (a.south) edge (onba.north);

    \end{tikzpicture}
    \caption{\subcapb}
\end{subfigure}


\newcommand{\xshift}{3cm}
\newcommand{\yshift}{-1cm}
\begin{subfigure}{0.49\columnwidth}
    \centering
    \begin{tikzpicture}[
            thick,
            every node/.style={
                    % shape=circle,
                    % minimum size=\csize,
                    % align=center,  
                    draw,
                    rounded corners,
                    minimum height=\minimumheight,  % Adjust as needed  
                    % minimum width=2cm,   % Adjust as needed  
                }
        ]

        \node[fill=caribbeangreen] (qaa) at (0, 0*\yshift) {$\ilgword{Q(a,a)}$};
        \node (qab) at (0, 1*\yshift) {$\ilgword{Q(a,b)}$};
        \node (qba) at (0, 2*\yshift) {$\ilgword{Q(b,a)}$};
        \node[fill=caribbeangreen] (qbb) at (0, 3*\yshift) {$\ilgword{Q(b,b)}$};
        \node (waa) at (0, 4*\yshift) {$\ilgword{W(a,a)}$};
        \node[fill=yellow] (wab) at (0, 5*\yshift) {$\ilgword{W(a,b)}$};
        \node[fill=yellow] (wba) at (0, 6*\yshift) {$\ilgword{W(b,a)}$};
        \node (wbb) at (0, 7*\yshift) {$\ilgword{W(b,b)}$};

        \node (oaa)[fill=pink] at (\xshift, 0.5*\yshift) {$\ilgword{o(a,a)}$};
        \node (oab) at (\xshift, 2.5*\yshift) {$\ilgword{o(a,b)}$};
        \node (oba) at (\xshift, 4.5*\yshift) {$\ilgword{o(b,a)}$};
        \node (obb)[fill=pink] at (\xshift, 6.5*\yshift) {$\ilgword{o(b,b)}$};

        \draw[draw=plta] (qaa.east) -- (oaa.west);
        \draw[draw=plta] (qab.east) -- (oab.west);
        \draw[draw=plta] (qba.east) -- (oba.west);
        \draw[draw=plta] (qbb.east) -- (obb.west);
        \draw[draw=pltb] (waa.east) -- (oaa.west);
        \draw[draw=pltb] (wab.east) -- (oab.west);
        \draw[draw=pltb] (wba.east) -- (oba.west);
        \draw[draw=pltb] (wbb.east) -- (obb.west);
    \end{tikzpicture}
    \caption{\subcapc}
\end{subfigure}
\begin{subfigure}{0.49\columnwidth}
    \centering
    \begin{tikzpicture}[
            thick,
            every node/.style={
                    % shape=circle,
                    % minimum size=\csize,
                    % align=center,  
                    draw,
                    rounded corners,
                    minimum height=\minimumheight,  % Adjust as needed  
                    % minimum width=2cm,   % Adjust as needed  
                }
        ]

        \node (qaa) at (0, 0*\yshift) {$\ilgword{Q(a,a)}$};
        \node[fill=caribbeangreen] (qab) at (0, 1*\yshift) {$\ilgword{Q(a,b)}$};
        \node[fill=caribbeangreen] (qba) at (0, 2*\yshift) {$\ilgword{Q(b,a)}$};
        \node (qbb) at (0, 3*\yshift) {$\ilgword{Q(b,b)}$};
        \node (waa) at (0, 4*\yshift) {$\ilgword{W(a,a)}$};
        \node[fill=yellow] (wab) at (0, 5*\yshift) {$\ilgword{W(a,b)}$};
        \node[fill=yellow] (wba) at (0, 6*\yshift) {$\ilgword{W(b,a)}$};
        \node (wbb) at (0, 7*\yshift) {$\ilgword{W(b,b)}$};

        \node (oaa) at (\xshift, 0.5*\yshift) {$\ilgword{o(a,a)}$};
        \node[fill=pink] (oab) at (\xshift, 2.5*\yshift) {$\ilgword{o(a,b)}$};
        \node[fill=pink] (oba) at (\xshift, 4.5*\yshift) {$\ilgword{o(b,a)}$};
        \node (obb) at (\xshift, 6.5*\yshift) {$\ilgword{o(b,b)}$};

        \draw[draw=plta] (qaa.east) -- (oaa.west);
        \draw[draw=plta] (qab.east) -- (oab.west);
        \draw[draw=plta] (qba.east) -- (oba.west);
        \draw[draw=plta] (qbb.east) -- (obb.west);
        \draw[draw=pltb] (waa.east) -- (oaa.west);
        \draw[draw=pltb] (wab.east) -- (oab.west);
        \draw[draw=pltb] (wba.east) -- (oba.west);
        \draw[draw=pltb] (wbb.east) -- (obb.west);
    \end{tikzpicture}
    \caption{\subcapd}
\end{subfigure}


==> figures/proofs/asnets-slg.tex <==
\newcommand\sizeforhopt{0.9cm}
\newcommand\yshifta{2.0}
\newcommand\yshiftb{0.5}
\newcommand\xshift{1.5}
\newcommand\textsize{\scriptsize}
  \begin{subfigure}{0.49\columnwidth}
    \centering
    \begin{tikzpicture}[square/.style={regular polygon,regular polygon sides=4}]
      \node[shape=rectangle,draw=black,minimum size=0.75*\sizeforhopt] (A1) at (0,0) {};
      \node[shape=rectangle,draw=black,minimum size=0.75*\sizeforhopt] (A2) at ([shift={(0,-\yshifta)}]A1) {};
      \node[shape=circle,draw=black,minimum size=0.75*\sizeforhopt] (P1) at ([shift={(\xshift,0)}]A1) {};
      \node[shape=circle,draw=black,minimum size=0.75*\sizeforhopt] (P2) at ([shift={(\xshift,0)}]A2) {};
      \node[shape=rectangle,draw=black,minimum size=0.75*\sizeforhopt] (A3) at ([shift={(\xshift,+\yshiftb)}]P1) {};
      \node[shape=rectangle,draw=black,minimum size=0.75*\sizeforhopt] (A4) at ([shift={(\xshift,-\yshiftb)}]P1) {};
      \node[shape=rectangle,draw=black,minimum size=0.75*\sizeforhopt] (A5) at ([shift={(\xshift,+\yshiftb)}]P2) {};
      \node[shape=rectangle,draw=black,minimum size=0.75*\sizeforhopt] (A6) at ([shift={(\xshift,-\yshiftb)}]P2) {};
      \node[shape=circle,draw=black,minimum size=0.75*\sizeforhopt] (G3) at ([shift={(2*\xshift,0)}]P1) {};
      \node[shape=circle,draw=black,minimum size=0.75*\sizeforhopt] (G4) at ([shift={(2*\xshift,0)}]P2) {};
      \node[shape=circle,draw=black,minimum size=0.6*\sizeforhopt] (G33) at (G3) {};
      \node[shape=circle,draw=black,minimum size=0.6*\sizeforhopt] (G44) at (G4) {};

      \node at (A1) {\textsize$a_1^{(1)}$};
      \node at (A2) {\textsize$a_2^{(1)}$};
      \node at (P1) {\textsize$p_1$};
      \node at (P2) {\textsize$p_2$};
      \node at (A3) {\textsize$a_3^{(1)}$};
      \node at (A4) {\textsize$a_4^{(1)}$};
      \node at (A5) {\textsize$a_5^{(1)}$};
      \node at (A6) {\textsize$a_6^{(1)}$};
      \node at (G3) {\textsize$g_3$};
      \node at (G4) {\textsize$g_4$};


      \path [-,draw=blue] (A1) edge (P1);
      % \path [<-,bend right] (A1) edge (P1);

      \path [-,draw=blue] (A2) edge (P2);
      % \path [<-,bend right] (A2) edge (P2);

      \path [-] (P1) edge (A3);
      % \path [<-,bend right] (P1) edge (A3);

      \path [-] (P1) edge (A4);
      % \path [-,bend right] (P1) edge (A4);
      
      \path [-] (P2) edge (A5);
      % \path [<-,bend right] (P2) edge (A5);
      
      \path [-] (P2) edge (A6);
      % \path [-,bend right] (P2) edge (A6);
      
      \path [-,draw=blue] (A3) edge (G3);
      % \path [<-,bend right] (A3) edge (G3);
      
      \path [-,draw=blue] (A4) edge (G3);
      % \path [-,bend right] (A4) edge (G3);

      \path [-,draw=blue] (A5) edge (G4);
      % \path [<-,bend right] (A5) edge (G4);

      \path [-,draw=blue] (A6) edge (G4);
      % \path [-,bend right] (A6) edge (G4);
    \end{tikzpicture}
    \caption{\slg{} of $P_1$.}
  \end{subfigure}
  \begin{subfigure}{0.49\columnwidth}
    \centering
    \begin{tikzpicture}[square/.style={regular polygon,regular polygon sides=4}]
      \node[shape=rectangle,draw=black,minimum size=0.75*\sizeforhopt] (A1) at (0,0) {};
      \node[shape=rectangle,draw=black,minimum size=0.75*\sizeforhopt] (A2) at ([shift={(0,-\yshifta)}]A1) {};
      \node[shape=circle,draw=black,minimum size=0.75*\sizeforhopt] (P1) at ([shift={(\xshift,0)}]A1) {};
      \node[shape=circle,draw=black,minimum size=0.75*\sizeforhopt] (P2) at ([shift={(\xshift,0)}]A2) {};
      \node[shape=rectangle,draw=black,minimum size=0.75*\sizeforhopt] (A3) at ([shift={(\xshift,+\yshiftb)}]P1) {};
      \node[shape=rectangle,draw=black,minimum size=0.75*\sizeforhopt] (A4) at ([shift={(\xshift,-\yshiftb)}]P1) {};
      \node[shape=rectangle,draw=black,minimum size=0.75*\sizeforhopt] (A5) at ([shift={(\xshift,+\yshiftb)}]P2) {};
      \node[shape=rectangle,draw=black,minimum size=0.75*\sizeforhopt] (A6) at ([shift={(\xshift,-\yshiftb)}]P2) {};
      \node[shape=circle,draw=black,minimum size=0.75*\sizeforhopt] (G3) at ([shift={(2*\xshift,0)}]P1) {};
      \node[shape=circle,draw=black,minimum size=0.75*\sizeforhopt] (G4) at ([shift={(2*\xshift,0)}]P2) {};
      \node[shape=circle,draw=black,minimum size=0.6*\sizeforhopt] (G33) at (G3) {};
      \node[shape=circle,draw=black,minimum size=0.6*\sizeforhopt] (G44) at (G4) {};

      \node at (A1) {\textsize$a_1^{(2)}$};
      \node at (A2) {\textsize$a_2^{(2)}$};
      \node at (P1) {\textsize$p_1$};
      \node at (P2) {\textsize$p_2$};
      \node at (A3) {\textsize$a_3^{(2)}$};
      \node at (A4) {\textsize$a_4^{(2)}$};
      \node at (A5) {\textsize$a_5^{(2)}$};
      \node at (A6) {\textsize$a_6^{(2)}$};
      \node at (G3) {\textsize$g_3$};
      \node at (G4) {\textsize$g_4$};

      \path [-,draw=blue] (A1) edge (P1);
      % \path [<-,bend right] (A1) edge (P1);

      \path [-,draw=blue] (A2) edge (P2);
      % \path [<-,bend right] (A2) edge (P2);

      \path [-] (P1) edge (A3.west);
      % \path [<-,bend right] (P1) edge (A3);

      \path [-] (P1) edge (A5.west);
      % \path [-,bend right] (P1) edge (A5);
      
      \path [-] (P2) edge (A4.west);
      % \path [-,bend left] (P2) edge (A4);
      
      \path [-] (P2) edge (A6.west);
      % \path [-,bend right] (P2) edge (A6);
      
      \path [-,draw=blue] (A3) edge (G3);
      % \path [<-,bend right] (A3) edge (G3);
      
      \path [-,draw=blue] (A4) edge (G3);
      % \path [-,bend right] (A4) edge (G3);

      \path [-,draw=blue] (A5) edge (G4);
      % \path [<-,bend right] (A5) edge (G4);

      \path [-,draw=blue] (A6) edge (G4);
      % \path [->,bend right] (A6) edge (G4);
    \end{tikzpicture}
    \caption{\slg{} of $P_2$.}
  \end{subfigure}

==> figures/proofs/ilg-muninn.tex <==
\newcommand{\xxshift}{1.25cm}
\newcommand{\yyshift}{2cm}
\newcommand{\csize}{0.8cm}
\newcommand{\descccsize}{\scriptsize}
\newcommand{\objectsize}{\descccsize}
\newcommand{\ilgword}[1]{\text{\descccsize{#1}}}
\newcommand{\objword}[1]{\text{\objectsize{#1}}}
\newcommand{\desccccc}{5cm}
\newcommand{\desccc}{6cm}
\newcommand{\anchor}{west}
\newcommand{\minimumheight}{1.5em}
\begin{subfigure}{0.49\columnwidth}
    \centering
    \begin{tikzpicture}[  
        thick,  
        every node/.style={  
            % shape=circle,
            % minimum size=\csize,
            % align=center,  
            draw,  
            rounded corners,  
            minimum height=\minimumheight,  % Adjust as needed  
            % minimum width=2cm,   % Adjust as needed  
        }  
    ]
    \node[fill=caribbeangreen] (onaa) at (-2.25*\xxshift,\yyshift) {
    $\ilgword{Q(a,a)}$
    };
    \node[fill=caribbeangreen] (onbb) at (-0.75*\xxshift,\yyshift) {
    $\ilgword{Q(b,b)}$
    };
    \node[fill=yellow] (onab) at ( 0.75*\xxshift,\yyshift) {
    $\ilgword{Q(a,b)}$
    };
    \node[fill=yellow] (onba) at ( 2.25*\xxshift,\yyshift) {
    $\ilgword{Q(b,a)}$
    };
    \node[fill=babyblue] (a) at (  -1.5*\xxshift,2*\yyshift) {
    $\objword{a}$
    };
    \node[fill=babyblue] (b) at (   1.5 *\xxshift,2*\yyshift) {
    $\objword{b}$
    };
    
    \path [-,draw=plta] (a.south) edge[bend left=15] (onaa.north);
    \path [-,draw=pltb] (a.south) edge[bend right=15] (onaa.north);
    \path [-,draw=plta] (b.south) edge[bend left=15] (onbb.north);
    \path [-,draw=pltb] (b.south) edge[bend right=15] (onbb.north);
    
    \path [-,draw=plta] (a.south) edge (onab.north);
    \path [-,draw=pltb] (b.south) edge (onab.north);
    
    \path [-,draw=plta] (b.south) edge (onba.north);
    \path [-,draw=pltb] (a.south) edge (onba.north);

    \end{tikzpicture}
    \caption{\subcapa}
\end{subfigure}
\begin{subfigure}{0.49\columnwidth}
    \centering
    \begin{tikzpicture}[  
        thick,  
        every node/.style={  
            % shape=circle,
            % minimum size=\csize,
            % align=center,  
            draw,  
            rounded corners,  
            minimum height=\minimumheight,  % Adjust as needed  
            % minimum width=2cm,   % Adjust as needed  
        }  
    ]
    \node[fill=aquamarine] (onab) at (-1.5*\xxshift,\yyshift) {
    $\ilgword{Q(a,b)}$
    };
    \node[fill=aquamarine] (onba) at ( 1.5*\xxshift,\yyshift) {
    $\ilgword{Q(b,a)}$
    };
    \node[fill=babyblue] (a) at (  -1.5*\xxshift,2*\yyshift) {
    $\objword{a}$
    };
    \node[fill=babyblue] (b) at (   1.5 *\xxshift,2*\yyshift) {
    $\objword{b}$
    };
    
    \path [-,draw=plta] (a.south) edge (onab.north);
    \path [-,draw=pltb] (b.south) edge (onab.north);
    
    \path [-,draw=plta] (b.south) edge (onba.north);
    \path [-,draw=pltb] (a.south) edge (onba.north);

    \end{tikzpicture}
    \caption{\subcapb}
\end{subfigure}
\begin{subfigure}{0.49\columnwidth}
    \centering
    \begin{tikzpicture}[  
        thick,  
        every node/.style={  
            % shape=circle,
            % minimum size=\csize,
            % align=center,  
            draw,  
            rounded corners,  
            minimum height=\minimumheight,  % Adjust as needed  
            % minimum width=2cm,   % Adjust as needed  
        }  
    ]
    \node[fill=gray!30] (onaa) at (-2.25*\xxshift,\yyshift) {
    $\ilgword{Q(a,a)}$
    };
    \node[fill=gray!30] (onbb) at (-0.75*\xxshift,\yyshift) {
    $\ilgword{Q(b,b)}$
    };
    \node[fill=gray!30] (onab) at ( 0.75*\xxshift,\yyshift) {
    $\ilgword{Q}_{\ilgword{g}}\ilgword{(a,b)}$
    };
    \node[fill=gray!30] (onba) at ( 2.25*\xxshift,\yyshift) {
    $\ilgword{Q}_{\ilgword{g}}\ilgword{(b,a)}$
    };
    \node[fill=gray!30] (a) at (  -1.5*\xxshift,2*\yyshift) {
    $\objword{a}$
    };
    \node[fill=gray!30] (b) at (   1.5 *\xxshift,2*\yyshift) {
    $\objword{b}$
    };
    
    \path [-,draw=plta] (a.south) edge[bend left=15] (onaa.north);
    \path [-,draw=pltb] (a.south) edge[bend right=15] (onaa.north);
    \path [-,draw=plta] (b.south) edge[bend left=15] (onbb.north);
    \path [-,draw=pltb] (b.south) edge[bend right=15] (onbb.north);
    
    \path [-,draw=pltc] (a.south) edge (onab.north);
    \path [-,draw=pltd] (b.south) edge (onab.north);
    
    \path [-,draw=pltc] (b.south) edge (onba.north);
    \path [-,draw=pltd] (a.south) edge (onba.north);

    \end{tikzpicture}
    \caption{\subcapc}
\end{subfigure}
\begin{subfigure}{0.49\columnwidth}
    \centering
    \begin{tikzpicture}[  
        thick,  
        every node/.style={  
            % shape=circle,
            % minimum size=\csize,
            % align=center,  
            draw,  
            rounded corners,  
            minimum height=\minimumheight,  % Adjust as needed  
            % minimum width=2cm,   % Adjust as needed  
        }  
    ]
    \node[fill=gray!30] (onab) at (-2.25*\xxshift,\yyshift) {
    $\ilgword{Q(a,b)}$
    };
    \node[fill=gray!30] (onba) at (-0.75*\xxshift,\yyshift) {
    $\ilgword{Q(b,a)}$
    };
    \node[fill=gray!30] (onabg) at ( 0.75*\xxshift,\yyshift) {
    $\ilgword{Q}_{\ilgword{g}}\ilgword{(a,b)}$
    };
    \node[fill=gray!30] (onbag) at ( 2.25*\xxshift,\yyshift) {
    $\ilgword{Q}_{\ilgword{g}}\ilgword{(b,a)}$
    };
    \node[fill=gray!30] (a) at (  -1.5*\xxshift,2*\yyshift) {
    $\objword{a}$
    };
    \node[fill=gray!30] (b) at (   1.5 *\xxshift,2*\yyshift) {
    $\objword{b}$
    };
    
    \path [-,draw=plta] (a.south) edge (onab.north);
    \path [-,draw=pltb] (b.south) edge (onab.north);
    \path [-,draw=plta] (b.south) edge (onba.north);
    \path [-,draw=pltb] (a.south) edge (onba.north);
    
    \path [-,draw=pltc] (a.south) edge (onabg.north);
    \path [-,draw=pltd] (b.south) edge (onabg.north);
    
    \path [-,draw=pltc] (b.south) edge (onbag.north);
    \path [-,draw=pltd] (a.south) edge (onbag.north);

    \end{tikzpicture}
    \caption{\subcapd}
\end{subfigure}


==> tables/data-coverage-template.tex <==
\begin{tabular}{cccrrrrrrrrrrr}
    \toprule
    Model & Data & Iterations & \header{Blocksworld} & \header{Childsnack} & \header{Ferry} & \header{Floortile} & \header{Miconic} & \header{Rovers} & \header{Satellite} & \header{Sokoban} & \header{Spanner} & \header{Transport} & \header{Sum} \\
    \midrule
    TO_REPLACE
    \bottomrule
\end{tabular}


==> tables/data-coverage.tex <==
\begin{tabular}{cccrrrrrrrrrrr}
    \toprule
    Model & Data & Iterations & \header{Blocksworld} & \header{Childsnack} & \header{Ferry} & \header{Floortile} & \header{Miconic} & \header{Rovers} & \header{Satellite} & \header{Sokoban} & \header{Spanner} & \header{Transport} & \header{Sum} \\
    \midrule
    $\gpr$& $\plans$ &1 &62 & 18 & 77 & 2 & 90 & 51 & 34 & 39 & 75 & 33 & 481\\& &2 &29 & 20 & 77 & 2 & 90 & 40 & 14 & 38 & 75 & 27 & 412\\& &3 &62 & 32 & 77 & 2 & 90 & 37 & 45 & 38 & 74 & 26 & 483\\& &4 &74 & 40 & 77 & 2 & 90 & 37 & 48 & 37 & 73 & 28 & 506\\\cmidrule{2-14}& $\states$ &1 &\worse{10} & \worse{13} & 77 & 2 & 90 & \worse{33} & \better{41} & 39 & \worse{63} & \better{50} & \worse{418}\\& &2 &\worse{23} & \worse{13} & 77 & 2 & 90 & \worse{31} & \better{36} & 37 & \worse{30} & \better{36} & \worse{375}\\& &3 &\better{71} & \worse{13} & 77 & 2 & 90 & \worse{31} & \worse{43} & 39 & \worse{30} & \better{39} & \worse{435}\\& &4 &\worse{27} & \worse{13} & 77 & 2 & 90 & \worse{32} & 48 & \better{39} & \worse{30} & \better{41} & \worse{399}\\\cmidrule{2-14}& $\both$ &1 &\better{66} & \worse{13} & 77 & 2 & 90 & \better{55} & \worse{31} & 39 & 75 & \better{39} & \better{487}\\& &2 &\better{90} & \worse{13} & 77 & 2 & 90 & \better{44} & \better{17} & 38 & \worse{51} & \worse{25} & \better{447}\\& &3 &\worse{39} & \worse{13} & 77 & 2 & 90 & \better{40} & \worse{40} & \worse{24} & \worse{68} & 27 & \worse{420}\\& &4 &\worse{59} & \worse{13} & 77 & 2 & 90 & \better{42} & \worse{40} & \worse{24} & \worse{69} & \worse{22} & \worse{438}\\\midrule$\svr$& $\plans$ &1 &49 & 18 & 77 & 2 & 90 & 52 & 59 & 39 & 75 & 33 & 494\\& &2 &35 & 21 & 77 & 2 & 90 & 43 & 49 & 38 & 75 & 31 & 461\\& &3 &67 & 32 & 77 & 2 & 90 & 36 & 54 & 38 & 74 & 30 & 500\\& &4 &70 & 39 & 77 & 2 & 90 & 35 & 57 & 38 & 73 & 30 & 511\\\cmidrule{2-14}& $\states$ &1 &\worse{8} & 18 & 77 & 1 & 90 & \worse{36} & \worse{35} & 39 & \better{78} & \better{50} & \worse{432}\\& &2 &\worse{8} & \worse{13} & 77 & 2 & 90 & \worse{31} & \worse{39} & 39 & \worse{31} & 32 & \worse{362}\\& &3 &\worse{48} & \worse{13} & 77 & 2 & 90 & \worse{30} & \worse{42} & 39 & \worse{54} & \better{35} & \worse{430}\\& &4 &\worse{54} & \worse{13} & 77 & 1 & 90 & \worse{31} & \worse{48} & 39 & \worse{56} & \better{37} & \worse{446}\\\cmidrule{2-14}& $\both$ &1 &\better{64} & 18 & 77 & 2 & 90 & \worse{47} & \worse{44} & 39 & 76 & \better{39} & \better{496}\\& &2 &\better{89} & \worse{15} & 77 & 2 & 90 & 42 & \worse{40} & 38 & \worse{72} & 31 & \better{496}\\& &3 &\worse{56} & \worse{18} & 77 & 2 & 90 & 36 & \worse{39} & 38 & \better{77} & \worse{27} & \worse{460}\\& &4 &\worse{61} & \worse{13} & 77 & 2 & 90 & 34 & \worse{40} & 38 & \better{76} & 30 & \worse{461}\\
    \bottomrule
\end{tabular}


==> tables/data-features-template.tex <==
\begin{tabular}{ccrrrrrrrrrr}
    \toprule
    Data & Iterations & \header{Blocksworld} & \header{Childsnack} & \header{Ferry} & \header{Floortile} & \header{Miconic} & \header{Rovers} & \header{Satellite} & \header{Sokoban} & \header{Spanner} & \header{Transport} \\
    \midrule
    TO_REPLACE
    \bottomrule
\end{tabular}


==> tables/data-features.tex <==
\begin{tabular}{ccrrrrrrrrrr}
    \toprule
    Data & Iterations & \header{Blocksworld} & \header{Childsnack} & \header{Ferry} & \header{Floortile} & \header{Miconic} & \header{Rovers} & \header{Satellite} & \header{Sokoban} & \header{Spanner} & \header{Transport} \\
    \midrule
    $\plans$ &1 &52 & 37 & 81 & 264 & 21 & 296 & 221 & 23 & 29 & 66\\&2 &347 & 84 & 344 & 1316 & 45 & 3402 & 2229 & 49 & 83 & 329\\&3 &2319 & 156 & 1199 & 3527 & 74 & 10409 & 8133 & 78 & 189 & 1215\\&4 &10444 & 251 & 3228 & 7616 & 108 & 23202 & 22155 & 110 & 350 & 3787\\\midrule$\states$ &1 &52 & 35 & 59 & 81 & 21 & 103 & 79 & 23 & 32 & 53\\&2 &385 & 75 & 221 & 521 & 45 & 634 & 396 & 49 & 106 & 254\\&3 &6359 & 139 & 668 & 2177 & 74 & 2161 & 1598 & 80 & 272 & 1048\\&4 &44233 & 234 & 1662 & 8574 & 108 & 5719 & 5475 & 118 & 550 & 4193\\\midrule$\both$ &1 &52 & 37 & 84 & 313 & 21 & 297 & 224 & 23 & 32 & 73\\&2 &385 & 85 & 355 & 1742 & 45 & 3533 & 2273 & 49 & 106 & 375\\&3 &7048 & 165 & 1275 & 5490 & 74 & 11332 & 8772 & 80 & 272 & 1535\\&4 &49952 & 283 & 3536 & 15783 & 108 & 26762 & 25787 & 118 & 550 & 5896\\
    \bottomrule
\end{tabular}


==> tables/data-template.tex <==
\begin{tabular}{crrrrrrrrrr}
    \toprule
    Data & \header{Blocksworld} & \header{Childsnack} & \header{Ferry} & \header{Floortile} & \header{Miconic} & \header{Rovers} & \header{Satellite} & \header{Sokoban} & \header{Spanner} & \header{Transport}\\
    \midrule
    TO_REPLACE
    \bottomrule
\end{tabular}


==> tables/data.tex <==
\begin{tabular}{crrrrrrrrrr}
    \toprule
    Data & \header{Blocksworld} & \header{Childsnack} & \header{Ferry} & \header{Floortile} & \header{Miconic} & \header{Rovers} & \header{Satellite} & \header{Sokoban} & \header{Spanner} & \header{Transport}\\
    \midrule
    $\plans$ & 1292 & 473 & 1368 & 3187 & 1630 & 1428 & 1158 & 2422 & 1204 & 735\\$\states$ & 10000 & 687 & 2316 & 1861 & 2832 & 1182 & 10000 & 2412 & 1578 & 2673\\$\both$ & 11292 & 1160 & 3684 & 5048 & 4462 & 2610 & 11158 & 4834 & 2782 & 3408\\
    \bottomrule
\end{tabular}


==> tables/gnn-wl-vertical.tex <==
\begin{tabular}{lrr}\toprule
 & $\gnn$ & $\gpr$ \\
\midrule Blocksworld & \bfseries 70 & \bfseries 70 \\
Childsnack & 26 & \bfseries 39 \\
Ferry & 70 & \bfseries 77 \\
Floortile & 0 & \bfseries 2 \\
Miconic & 89 & \bfseries 90 \\
Rovers & 26 & \bfseries 36 \\
Satellite & 33 & \bfseries 57 \\
Sokoban & 33 & \bfseries 38 \\
Spanner & 49 & \bfseries 73 \\
Transport & \bfseries 35 & 30 \\
\midrule Sum & 431 & \bfseries 512 \\
\bottomrule\end{tabular}


==> tables/gnn-wl.tex <==
\begin{tabular}{crrrrrrrrrrr}
    \toprule
    Model & \header{Blocksworld} & \header{Childsnack} & \header{Ferry} & \header{Floortile} & \header{Miconic} & \header{Rovers} & \header{Satellite} & \header{Sokoban} & \header{Spanner} & \header{Transport} & \header{Sum} \\
    \midrule
    \ifSVR
        GNN & \bfseries 70 & 26 & 70 & 0 & 89 & 26 & 33 & 33 & 49 & \bfseries 35 & 431 \\
        SVR & \bfseries 70 & \bfseries 39 & \bfseries 77 & \bfseries 2 & \bfseries 90 & \bfseries 35 & \bfseries 57 & \bfseries 38 & \bfseries 73 & 30 & \bfseries 511 \\
    \else
        GNN & 70 & 26 & 70 & 0 & 89 & 26 & 33 & 33 & 49 & \bfseries 35 & 431 \\
        GPR & \bfseries 74 & \bfseries 40 & \bfseries 77 & \bfseries 2 & \bfseries 90 & \bfseries 37 & \bfseries 48 & \bfseries 36 & \bfseries 73 & 28 & \bfseries 505 \\
    \fi
    \bottomrule
\end{tabular}


==> tables/planning_graphs_literature.tex <==
\small
\newcommand{\colWidth}{1.25cm}
\newcolumntype{C}[1]{>{\centering\arraybackslash}p{#1}}
\begin{tabularx}{\textwidth}{l C{\colWidth} C{\colWidth} C{\colWidth} X}
    \toprule
    Graph/Planner & \makecell{Node \\ Feat.} & \makecell{Edge \\ Feat.} & \makecell{Digraph} & Original Purpose/Learning Target \\
    \midrule
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    GraphPlan & 
    Yes & 
    Yes & 
    Yes & 
    planning algorithm~\cite{blum.furst.1997} \\
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    CG & 
    No & 
    No & 
    Yes & 
    CG heuristic~\cite{helmert.2004} \\
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    DTG & 
    No & 
    No & 
    Yes & 
    CG heuristic~\cite{helmert.2004} \\
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    Justif. Graph & 
    No & 
    Yes & 
    Yes & 
    LM-cut heuristic~\cite{helmert.domshlak.2009} \\
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    FDR-PDG & 
    Yes & 
    No & 
    No & 
    symmetries~\cite{pochter.etal.2011} \\
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    STRIPS-PDG & 
    Yes & 
    Yes & 
    Yes & 
    symmetries~\cite{shleyfman.etal.2015} \\
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    Gaif. Graphs & 
    No &
    No &
    Yes &
    lifted heuristics~\cite{horcik.fiser.2023} \\
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    ASG & 
    Yes & 
    No & 
    Yes & 
    symmetries~\cite{sievers.etal.2019} \\
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    Object Graphs &
    Yes &
    No &
    No &
    symmetries~\cite{drexler.etal.2024a} \\
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    \midrule
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    ASNets &
    Yes & 
    Yes & 
    Yes & 
    policy~\cite{toyer.etal.2018,toyer.etal.2020} \\
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    STRIPS-HGN &
    Yes & 
    Yes & 
    Yes & 
    domain-indep. heuristic~\cite{shen.etal.2020} \\
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    PLOI &
    Yes & 
    Yes & 
    Yes & 
    object importance~\cite{silver.etal.2021} \\
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    Muninn &
    No &
    Yes &
    Yes &
    value function~\cite{staahlberg.etal.2022} \\
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    GOOSE(SLG) &
    Yes &
    Yes &
    No &
    domain-indep. heuristic~\cite{chen.etal.2024} \\
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    GOOSE(FLG) &
    Yes &
    Yes &
    No &
    domain-indep. heuristic~\cite{chen.etal.2024} \\
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    GOOSE(LLG) &
    Yes &
    Yes &
    No &
    domain-indep. heuristic~\cite{chen.etal.2024} \\
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    GOOSE(ILG) &
    Yes &
    Yes &
    No &
    heuristic~\cite{chen.etal.2024a} \\
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    various graphs &
    Yes &
    Yes &
    No &
    expressivity checking~\cite{horcik.sir.2024} \\
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    \bottomrule
\end{tabularx}


==> tables/wl-best-template.tex <==
\begin{tabular}{rrrrrrrrrrr}
    \toprule
    \header{Blocksworld} & \header{Childsnack} & \header{Ferry} & \header{Floortile} & \header{Miconic} & \header{Rovers} & \header{Satellite} & \header{Sokoban} & \header{Spanner} & \header{Transport} & \header{Sum} \\
    \midrule
    TO_REPLACE
    \bottomrule
\end{tabular}


==> tables/wl-best.tex <==
\begin{tabular}{rrrrrrrrrrr}
    \toprule
    \header{Blocksworld} & \header{Childsnack} & \header{Ferry} & \header{Floortile} & \header{Miconic} & \header{Rovers} & \header{Satellite} & \header{Sokoban} & \header{Spanner} & \header{Transport} & \header{Sum} \\
    \midrule
    86 & 40 & 77 & 6 & 90 & 54 & 59 & 39 & 76 & 53 & 580\\
    \bottomrule
\end{tabular}


==> tables/wl-configurations-template.tex <==
\begin{tabular}{ccrrrrrrrrrrr}
    \toprule
    Model & Iterations & \header{Blocksworld} & \header{Childsnack} & \header{Ferry} & \header{Floortile} & \header{Miconic} & \header{Rovers} & \header{Satellite} & \header{Sokoban} & \header{Spanner} & \header{Transport} & \header{Sum} \\
    \midrule
    TO_REPLACE
    \bottomrule
\end{tabular}


==> tables/wl-configurations.tex <==
\begin{tabularx}{\textwidth}{lc*{11}{Y}}
    \toprule
    Model & Iterations & \header{Blocksworld} & \header{Childsnack} & \header{Ferry} & \header{Floortile} & \header{Miconic} & \header{Rovers} & \header{Satellite} & \header{Sokoban} & \header{Spanner} & \header{Transport} & \header{Sum} \\
    \midrule
    $\hff$ & --& 28 & 26 & 68 & 12 & 90 & 34 & 65 & 36 & 30 & 41 & 430 \\
    \lama{} & --& 61 & 35 & 68 & 11 & 90 & 67 & 89 & 40 & 30 & 66 & 557 \\
    \midrule
    $\gpr$ & 1 & 62 & 18 & \first{77} & 2 & \first{90} & \third{51} & 34 & \first{39} & \second{75} & 33 & 481\\ & 2 & 29 & 20 & \first{77} & 2 & \first{90} & 40 & 14 & \second{38} & \second{75} & 27 & 412\\ & 3 & 62 & 32 & \first{77} & 2 & \first{90} & 37 & 45 & \second{38} & \third{74} & 26 & 483\\ & 4 & 74 & \first{40} & \first{77} & 2 & \first{90} & 37 & 48 & \third{37} & 73 & 28 & 506\\\midrule$\svr$ & 1 & 49 & 18 & \first{77} & 2 & \first{90} & \second{52} & \first{59} & \first{39} & \second{75} & 33 & 494\\ & 2 & 35 & 21 & \first{77} & 2 & \first{90} & 43 & 49 & \second{38} & \second{75} & 31 & 461\\ & 3 & 67 & 32 & \first{77} & 2 & \first{90} & 36 & \third{54} & \second{38} & \third{74} & 30 & 500\\ & 4 & 70 & \second{39} & \first{77} & 2 & \first{90} & 35 & \second{57} & \second{38} & 73 & 30 & \third{511}\\\midrule$\gpc$ & 1 & 59 & 36 & \first{77} & \first{6} & \first{90} & 39 & \oom{} & \first{39} & \second{75} & \third{45} & \notAllTried{466}\\ & 2 & \third{83} & \third{37} & \first{77} & \second{4} & \first{90} & 39 & \oom{} & \first{39} & 59 & 33 & \notAllTried{461}\\ & 3 & 82 & 35 & \first{77} & \third{3} & \first{90} & 40 & \oom{} & \first{39} & 56 & 37 & \notAllTried{459}\\ & 4 & \first{86} & 34 & \first{77} & 2 & \first{90} & 39 & \oom{} & \second{38} & 53 & 31 & \notAllTried{450}\\\midrule$\svm$ & 1 & 57 & 30 & \first{77} & \first{6} & \first{90} & 39 & 39 & \first{39} & \first{76} & \second{47} & 500\\ & 2 & 82 & 31 & \first{77} & \third{3} & \first{90} & 41 & 35 & \second{38} & \first{76} & 32 & 505\\ & 3 & 82 & \third{37} & \first{77} & 2 & \first{90} & 46 & 32 & \second{38} & \second{75} & 34 & \second{513}\\ & 4 & 78 & 33 & \first{77} & 2 & \first{90} & 41 & \oom{} & \second{38} & \third{74} & 31 & \notAllTried{464}\\\midrule$\lp$ & 1 & 24 & 18 & \first{77} & \first{6} & \first{90} & \first{54} & 34 & \first{39} & \second{75} & \first{53} & 470\\ & 2 & 79 & 18 & \first{77} & \second{4} & \first{90} & \second{52} & 46 & \first{39} & \third{74} & 32 & \third{511}\\ & 3 & \third{83} & 18 & \first{77} & \third{3} & \first{90} & 50 & 51 & \first{39} & \third{74} & 35 & \first{520}\\ & 4 & 81 & 18 & \first{77} & 2 & \first{90} & \second{52} & \oom{} & \first{39} & 73 & 34 & \notAllTried{466}\\\midrule$\mip$ & 1 & 24 & 18 & \first{77} & \third{3} & \first{90} & \second{52} & 29 & \first{39} & \second{75} & \second{47} & 454\\ & 2 & 75 & 18 & \first{77} & \oom{} & \first{90} & \third{51} & \oom{} & \first{39} & \third{74} & 37 & \notAllTried{461}\\ & 3 & \second{85} & 18 & \first{77} & \oom{} & \first{90} & \third{51} & \oom{} & \first{39} & \first{76} & \oom{} & \notAllTried{436}\\ & 4 & 49 & 18 & \first{77} & \oom{} & \first{90} & \oom{} & \oom{} & \first{39} & \first{76} & \oom{} & \notAllTried{349}\\
    \bottomrule
\end{tabularx}


==> tables/wl-group-iterations-template.tex <==
\begin{tabular}{crrrrrrrrrrr}
    \toprule
    Iterations & \header{Blocksworld} & \header{Childsnack} & \header{Ferry} & \header{Floortile} & \header{Miconic} & \header{Rovers} & \header{Satellite} & \header{Sokoban} & \header{Spanner} & \header{Transport} & \header{Sum} \\
    \midrule
    TO_REPLACE
    \bottomrule
\end{tabular}


==> tables/wl-group-iterations.tex <==
\begin{tabular}{crrrrrrrrrrr}
    \toprule
    Iterations & \header{Blocksworld} & \header{Childsnack} & \header{Ferry} & \header{Floortile} & \header{Miconic} & \header{Rovers} & \header{Satellite} & \header{Sokoban} & \header{Spanner} & \header{Transport} & \header{Sum} \\
    \midrule
    1 & 62 & \third{36} & \first{77} & \first{6} & \first{90} & \first{54} & \first{59} & \first{39} & \first{76} & \first{53} & \second{552}\\2 & \third{83} & \second{37} & \first{77} & \second{4} & \first{90} & \second{52} & 49 & \first{39} & \first{76} & \second{37} & 544\\3 & \second{85} & \second{37} & \first{77} & \third{3} & \first{90} & \third{51} & \third{54} & \first{39} & \first{76} & \second{37} & \third{549}\\4 & \first{86} & \first{40} & \first{77} & 2 & \first{90} & \second{52} & \second{57} & \first{39} & \first{76} & \third{34} & \first{553}\\
    \bottomrule
\end{tabular}


==> tables/wl-group-model-template.tex <==
\begin{tabular}{crrrrrrrrrrr}
    \toprule
    Model & \header{Blocksworld} & \header{Childsnack} & \header{Ferry} & \header{Floortile} & \header{Miconic} & \header{Rovers} & \header{Satellite} & \header{Sokoban} & \header{Spanner} & \header{Transport} & \header{Sum} \\
    \midrule
    TO_REPLACE
    \bottomrule
\end{tabular}


==> tables/wl-group-model.tex <==
\begin{tabular}{crrrrrrrrrrr}
    \toprule
    Model & \header{Blocksworld} & \header{Childsnack} & \header{Ferry} & \header{Floortile} & \header{Miconic} & \header{Rovers} & \header{Satellite} & \header{Sokoban} & \header{Spanner} & \header{Transport} & \header{Sum} \\
    \midrule
    $\gpr$ & 74 & \first{40} & \first{77} & \third{2} & \first{90} & \third{51} & \third{48} & \first{39} & \second{75} & 33 & 529\\$\svr$ & 70 & \second{39} & \first{77} & \third{2} & \first{90} & \second{52} & \first{59} & \first{39} & \second{75} & 33 & \third{536}\\$\gpc$ & \first{86} & \third{37} & \first{77} & \first{6} & \first{90} & 40 & \oom{} & \first{39} & \second{75} & \third{45} & \notAllTried{495}\\$\svm$ & 82 & \third{37} & \first{77} & \first{6} & \first{90} & 46 & 39 & \first{39} & \first{76} & \second{47} & \second{539}\\$\lp$ & \third{83} & 18 & \first{77} & \first{6} & \first{90} & \first{54} & \second{51} & \first{39} & \second{75} & \first{53} & \first{546}\\$\mip$ & \second{85} & 18 & \first{77} & \second{3} & \first{90} & \second{52} & 29 & \first{39} & \first{76} & \second{47} & 516\\
    \bottomrule
\end{tabular}


==> tables/wl-groups-template.tex <==
\begin{tabular}{crrrrrrrrrrr}
    \toprule
     & \header{Blocksworld} & \header{Childsnack} & \header{Ferry} & \header{Floortile} & \header{Miconic} & \header{Rovers} & \header{Satellite} & \header{Sokoban} & \header{Spanner} & \header{Transport} & \header{Sum} \\
    \midrule
    TO_REPLACE_1
    \midrule
    TO_REPLACE_2
    \midrule
    & 
    TO_REPLACE_3
    \bottomrule
\end{tabular}


==> tables/wl-groups.tex <==
\begin{tabularx}{\textwidth}{l*{11}{Y}}
    \toprule
     & \header{Blocksworld} & \header{Childsnack} & \header{Ferry} & \header{Floortile} & \header{Miconic} & \header{Rovers} & \header{Satellite} & \header{Sokoban} & \header{Spanner} & \header{Transport} & \header{Sum} \\
     \midrule
     $\hff$ & 28 & 26 & 68 & 12 & 90 & 34 & 65 & 36 & 30 & 41 & 430 \\
     \lama{} & 61 & 35 & 68 & 11 & 90 & 67 & 89 & 40 & 30 & 66 & 557 \\
    \midrule
    $\gpr$ & 74 & \first{40} & \first{77} & \third{2} & \first{90} & \third{51} & \third{48} & \first{39} & \second{75} & 33 & 529\\$\svr$ & 70 & \second{39} & \first{77} & \third{2} & \first{90} & \second{52} & \first{59} & \first{39} & \second{75} & 33 & \third{536}\\$\gpc$ & \first{86} & \third{37} & \first{77} & \first{6} & \first{90} & 40 & \oom{} & \first{39} & \second{75} & \third{45} & \notAllTried{495}\\$\svm$ & 82 & \third{37} & \first{77} & \first{6} & \first{90} & 46 & 39 & \first{39} & \first{76} & \second{47} & \second{539}\\$\lp$ & \third{83} & 18 & \first{77} & \first{6} & \first{90} & \first{54} & \second{51} & \first{39} & \second{75} & \first{53} & \first{546}\\$\mip$ & \second{85} & 18 & \first{77} & \second{3} & \first{90} & \second{52} & 29 & \first{39} & \first{76} & \second{47} & 516\\
    \midrule
    1 & 62 & \third{36} & \first{77} & \first{6} & \first{90} & \first{54} & \first{59} & \first{39} & \first{76} & \first{53} & \second{552}\\2 & \third{83} & \second{37} & \first{77} & \second{4} & \first{90} & \second{52} & 49 & \first{39} & \first{76} & \second{37} & 544\\3 & \second{85} & \second{37} & \first{77} & \third{3} & \first{90} & \third{51} & \third{54} & \first{39} & \first{76} & \second{37} & \third{549}\\4 & \first{86} & \first{40} & \first{77} & 2 & \first{90} & \second{52} & \second{57} & \first{39} & \first{76} & \third{34} & \first{553}\\
    \midrule
    $\max_{\text{domain}}$ & 86 & 40 & 77 & 6 & 90 & 54 & 59 & 39 & 76 & 53 & 580\\
    $\max_{\text{task}}$ & 90 & 60 & 77 & 6 & 90 & 58 & 63 & 39 & 79 & 57 & 619 \\
    \bottomrule
\end{tabularx}

